A Survey of Multi-Access Edge Computing in 5G and Beyond: Fundamentals, Technology Integration, and State-of-the-Art

Driven by the emergence of new compute-intensive applications and the vision of the Internet of Things (IoT), it is foreseen that the emerging 5G network will face an unprecedented increase in traffic volume and computation demands. However, end users mostly have limited storage capacities and finite processing capabilities, thus how to run compute-intensive applications on resource-constrained users has recently become a natural concern. Mobile edge computing (MEC), a key technology in the emerging fifth generation (5G) network, can optimize mobile resources by hosting compute-intensive applications, process large data before sending to the cloud, provide the cloud computing capabilities within the radio access network (RAN) in close proximity to mobile users, and offer context-aware services with the help of RAN information. Therefore, MEC enables a wide variety of applications, where the real-time response is strictly required, e.g., driverless vehicles, augmented reality, robotics, and immerse media. Indeed, the paradigm shift from 4G to 5G could become a reality with the advent of new technological concepts. The successful realization of MEC in the 5G network is still in its infancy and demands for constant efforts from both academic and industry communities. In this survey, we first provide a holistic overview of MEC technology and its potential use cases and applications. Then, we outline up-to-date researches on the integration of MEC with the new technologies that will be deployed in 5G and beyond. We also summarize testbeds and experimental evaluations, and open source activities, for edge computing. We further summarize lessons learned from state-of-the-art research works as well as discuss challenges and potential future directions for MEC research.

==> HetNet.tex <==
\section{MEC in Heterogeneous Cloud Radio Access Networks}
\label{Sec:HetNet_MEC}

\begin{figure*} [ht]
	\centering
	\includegraphics[scale=0.55]{./Images/HeterogeneousNetworks.pdf}
	\caption{Heterogeneous Networks Architecture \cite{Chan2010Pivotal}.}
	\label{Fig:HeterogeneousNetworks}
\end{figure*}

\subsection{Fundamentals of HetNets}
\label{SubSec:Fundamentals_HetNet}
In response to an unprecedented increase in network traffic volume and the massive number of connected devices, network densification has become the cornerstone of the 5G networks, where more base stations and access points are added and spatial spectrum reuse is exploited. HetNet is defined as an integration of higher-tier macrocells and lower-tier small cells, for example, picocells, femtocells, and relay nodes as illustrated in Fig.~\ref{Fig:HeterogeneousNetworks}. In other words, HetNets are created by integrating small cells into the existing cellular networks to provide seamless device-to-core network connectivity \cite{Ngo2014Architectures}. Nodes in HetNets can adopt and employ different access technologies over both licensed and unlicensed bands, for example, one node can use LTE as the access technology while the other uses WiFi. According to \cite{Ngo2014Architectures}, the minimum requirements of HetNet architectures are as follows:
\begin{itemize}
	\item \textit{Scalability}: Since many thousands of small cells can be deployed in one single network, the new architecture should support sufficient scalability.
	\item \textit{Transparent integration}: This requirement means that the deployment of small cells to the existing cellular networks should be easy and transparent.
	\item \textit{Security}: Small cells are usually deployed in insecure environments, thus the new architecture should provide sufficient security for both mobile networks and users. 
	\item \textit{Limited backhaul capacity}: With the increasing network densification, deploying all small cells with wired backhaul
	would not be a feasible and cost-effective solution due to
	fiber backhaul link installation obstacles \cite{Pham2018Mobile}. This has motivated the adoption of wireless backhaul for small cells so as to enable small cells receiving from and sending data traffic to macro base stations (MBSs) in a wireless fashion. 
\end{itemize}

HetNets have been developed because of many reasons. Main benefits of HetNets are summarized as follows \cite{Chandrasekhar2008Femtocell}:
\begin{itemize}
	\item \textit{Better coverage and capacity}: As more small cells are integrated into HetNets, the distance between transmitters and receivers becomes shorter. Therefore, HetNets can prolong battery life and achieve higher signal-to-interference-plus-noise ratio (SINR), thus resulting in larger capacity \cite{Chandrasekhar2008Femtocell}. The larger the number of small cells is, the higher the number of users can be served in an area with the same spectrum, hence, HetNets can improve the spectral efficiency or network capacity. 
	\item \textit{Improved macrocell reliability}: By means of traffic offloading, macrocells can reserve their resources to provide better quality to their serving users. 
	\item \textit{Cost benefits}: The deployment of small cells can reduce the operational expenditure and capital expenditure of cellular network operators \cite{Mugume2015Spectral}. According to \cite{Heath2007Picocells}, expenses scale from \$60000/year per macrocell to \$200/year per femtocell.
	\item \textit{Reduced subscriber turnover}: When small cells are available, mobile users are not limited by poor coverage of macrocells, thus removing the tendency to keep the wireline connection or switch to other MNOs. 
\end{itemize} 

Recently, in the context of 5G networks, HetNet is considered under the terms of dense network, hyper-dense network, extremely-dense network, and ultra-dense network \cite{Kamel2016Ultra}. Here, the term ``dense" refers to an extreme point, where the number deployed BSs becomes higher than the number of active users. There are several points that make dense HetNet different from regular HetNet as well as traditional networks \cite{Lopez2015Towards}. Firstly, the density of users is larger than that of BSs, thus it is possible that a mobile user is under the coverage of multiple small-eNBs. In such a scenario, user association is required for users to determine the suitable eNB to associate with and plays an important role in optimizing the operation and improving the performance of dense HetNets. However, an adverse consequence of network densification is frequent handover, which significantly affects the instant performance \cite{Sung2013Predictive}. More specifically, each handover necessitates the need for information exchange between users and eNBs, and the connection can be dropped if the handover operation fails \cite{Hartmann2017Radio}. Secondly, forwarding and receiving (i.e., backhauling) massive traffic from small-eNBs to macro-eNBs and over the core network is challenging. Actually, backhaul for small cells consists of wired and wireless backhauling \cite{Pham2018Mobile}. Choosing these backhaul solutions would depend on several factors, such as the cost of implementing backhaul connections, traffic load intensity, latency, and service requirements of mobile users. As small cells are densely deployed in 5G networks, implementing wired backhaul for a great number of small cells would not be affordable or even feasible. In this context, wireless backhaul has emerged as a viable solution and has received enormous attention from the academic and industry communities \cite{Liu2016Joint, Nie2017Forward, Nguyen2017Centralized}. Thirdly, interference is a limiting factor in dense HetNets. As network densification increases, the distance among small cells becomes smaller but the interference becomes more severe. Compared to traditional networks, new types of interference are introduced in (dense) HetNets: macro- to small cell interference, small- to small cell interference, and small- to macrocell interference. As the fundamental limits of capacity and achievable data rates mainly depend on the received interference, new and efficient interference management schemes, e.g., small-eNB on/off and frequency reuse, are of importance for guaranteeing the network performance. Finally, more sophisticated and practical propagation models are required in dense HetNets \cite{Lopez2015Towards}. While users and eNBs are positioned in 2D planes in traditional networks and regular HetNets, they can be distributed over both the horizontal space and vertical dimension in dense HetNets, such as in urban areas with many skyscrapers. In such a case, mobile users are close enough to the targeted eNBs to establish the line-of-sight (LoS) connections. On the other hand, the received signal at mobile users can be largely dominated by the LoS interfering links. This makes the single-slope path loss model used in regular HetNets not suitable for propagation modeling in dense HetNets \cite{Zhang2015Downlink}. 

In order to model, optimize, and analyze dense HetNets, several performance metrics have been used in the existing literature, including SINR distribution/outage probability, rate coverage and rate outage, average spectral efficiency (SE), area SE, network throughput, energy efficiency, and fairness and priorities. Several techniques can be used to address the challenges of dense HetNets, e.g., centralized optimization, stochastic geometry, game theory, and machine learning. For more information on these metrics and mathematical tools, we invite the reader to further refer to the following references \cite{Kamel2016Ultra, Liu2016UserAssociation, Teng2018Resource, Fan2018Machine}. 

\subsection{Motivations and Challenges}
\label{SubSec:Motivation_HetNet}
While the concept of HetNets has been introduced for almost a decade, the concept of edge computing and MEC has been recently developed by ETSI since 2014. On the one hand, the main idea behind HetNets is to offload traffic from macrocells to small cells so as to reduce the congestion in macrocells as well as enhancing the user QoS and the network performance. On the other hand, MEC is to move computing capabilities and storage resources from the core to the network edge. Despite different developing reasons and goals, HetNet and MEC share various similarities and complement each other. First, both the concepts aim at bringing manageable resources close to end users, wireless radio resources with HetNets and computing resources with MEC. Two terms, \textit{traffic offloading} and \textit{computation offloading}, are very common in HetNet and MEC. Specifically, the former indicates the offloading process of traffic data from higher-tier macrocells to lower-tier small cells, and the latter implies a typical use case of MEC as computing tasks can be offloaded from local resource-poor users to remote MEC servers. Next, the popularity of smart phones and the unprecedented increase in traffic volume have motivated the prosperity of many emerging services and applications, which usually have strict requirements of compute-intensive, delay-sensitive, ultra-reliable, and high-data-rate. The combination of MEC and HetNet is unavoidable to comply with these requirements. We consider the IoT with several thousands of users with low-latency and compute-intensive applications as an example. An MEC server that is collocated with the macro-eNB would not be able to serve a very large number of IoT devices due to the fact that MEC servers have typically limited computing resources. Moreover, because of small size and insufficient battery energy, many IoT devices are tiny and not able to directly connect with the macro-eNB collocated MEC server. In such a case, the presence of small cells can not only move storage and computing resources closer to users, but also decrease the transmission range between IoT devices and MEC servers, thus supporting the direct connection and reducing the latency. Thirdly, merging MEC with the dense deployment of small-eNBs is a potential solution for using cloud functionalities in a real-proximity and low-latency manner. Due to the sparse radio resources, offloading too many computation tasks to the single macro MEC server is very inefficient. If there is no available radio resource, users must wait until a resource block is available to offload their computation tasks. The integration of computing capabilities into small-eNBs can increase the number of offloading users compared to traditional network settings, where MEC servers are merely collocated with macro-eNBs. Finally, integrating MEC into HetNet promotes the design of heterogeneous MEC (Het-MEC) systems \cite{Mao2017_aSurveyMEC}, where MEC servers with various communication and computation capabilities are placed at different tiers, i.e., macro-MEC and small-MEC servers. It is worth noting that MEC and MCC are two complementary technologies in the sense that the centralized cloud can provide huge computation resources but long latency while the distributed MEC can achieve lower latency and higher reliability but limited computing capabilities. In such kinds of multi-tier and hierarchical MEC systems, mobile users can exploit various computing servers with heterogeneous computation capabilities, thus being able to run more complicated applications, and MEC servers at the same, even different, tiers can collaborate to execute enormous computations and reduce the peak computation workloads so as to improve the computing performance \cite{Pham2018MEC_HetNet}. 

With the concept of network densification and recent advancements in computing hardware, there may exist multiple MEC servers, where each one is connected to and collocated with a small-eNB. Very recently, few works have considered the existence of multiple servers in MEC networks for various problems, such as jointly adjusting the computational speed and offloading subtasks of a single user to multiple MEC servers \cite{Dinh2017Offloading}, joint computation offloading and resource allocation in multi-server MEC networks \cite{Tran2017Collaborative, Pham2018Decentralized}, and the minimum number of active MEC server \cite{Ranadheera2018Computation}. Compared with the single-server MEC network, MEC with multiple MEC servers could provide enormous benefits as follows \cite{Tran2017Collaborative, Pham2018Decentralized}:
\begin{itemize}
	\item Due to the economic and scalable deployments, the MEC server usually has limited computation resources. In addition, it is predicted that the mobile traffic will increase 1000 times over the next decade and the number of connected users will reach 50 billion in 2020, the single MEC server will likely become seriously overloaded. In contrast, mobile users can offload their computations to the best among several available MEC servers, thus reducing the burden of computation from the single MEC server.
	\item Under the coverage of multiple MEC servers, each user can offload the computation task to the MEC server with more favourable channel gain and computation capability. Therefore, mobile users can save the transmission energy consumption (thus the total energy consumption) and shorten the execution latency.
	\item In the case of partial offloading, each user can divide its computation task into several parts and offload them to different MEC servers, thereby reducing the execution latency. MEC servers can coordinate to exchange information to reduce ICI among offloading users across neighbouring MEC servers and improve the resource allocation efficiency. Moreover, collaboration among different MEC servers can help potentially increase the cluster resources, so affordable to support applications with higher computation requirements. 
\end{itemize} 

In addition to extra benefits, there exist several challenges in Het-MEC systems that can be induced by the characteristics of dense HetNets, features of MEC, uncertainty of user locations, and running applications and services. In the following, the major challenges of Het-MEC systems are discussed \cite{Pham2018Decentralized, Oo2017Offloading, Teng2018Resource}.
\begin{itemize}
	\item The availability of multiple MEC servers and/or small-eNBs makes the offloading decision problem particularly complex. Each MU must decide that \textit{i}) what is the optimal operation mode: \textit{offload} or \textit{not offload} and \textit{ii}) which small-eNB and MEC server should be selected to associate with and offload to, respectively, such that the achieved performance is maximized while the constraints on resource allocation and computation tasks are satisfied. 
	\item Due to the existence of ICI, the resource allocation problem in Het-MEC networks is much more challenging than that in homogeneous MEC systems \cite{Tran2017Collaborative}. To mitigate this effect, the spectrum resource within each cell can be divided into orthogonal subchannels, which should be efficiently allocated to mobile users (i.e., which subchannel a user should use to offload its computation task to the MEC server). The network performance can be further improved by jointly optimizing the subchannel assignment and adjusting the transmit power of mobile users.   
	\item On the one hand, it is foreseeable that a massive number of MEC servers will be distributedly deployed in the near future, which can be distinctly different in sizes (computing units) and configurations (computational speeds). On the other hand, the association between users and MEC servers is greatly dependent on the deployment locations of the MEC servers, e.g., a specific area may be densified by a large number of MEC servers while only one server is deployed in other areas. Mobile users may run applications and services with different priorities and security levels, e.g., some services can only run in private MEC servers due to security consideration. Moreover, computation tasks may be different in input data size, computation workload, and execution deadline. As a result, the joint resource allocation problem should take into account the above properties and characteristics.  
	\item In terms of resource allocation, the computational complexity arises as one of the most key issues. Unlike traditional MEC systems, where typically there is one MEC server per cell and several tens of mobile users, in dense Het-MEC systems, the number of variables needed to be optimized increases exponentially with the number of active users, deployed eNBs, MEC servers, and great deal resources. Various types of resources are considered in dense Het-MEC systems including not only conventional wireless resources (e.g., subchannel, transmit power, time, and space) but also newly introduced ones (e.g., backhaul spectrum, harvested energy, computing capabilities, and caching storage). The major challenges of dense Het-MEC systems are user association, computation offloading, interference management, and resource allocation. More importantly, these problems are tightly coupled and must be solved simultaneously. In such dense Het-MEC systems, how to design efficient algorithms in the distributed fashion with low-complexity and small signaling overhead is challenging, thus demanding enormous efforts from the communities in the future.  
\end{itemize}

\subsection{State of the Art}
\label{SubSec:State_of_the_Art_HetNet}
The majority of the existing studies have focused on single-server MEC networks. Typical network settings are \textit{i}) single-cell networks, where an MEC server is integrated into the BS and \textit{ii}) single-server MEC HetNets, where multiple small cells are overlaid within a macrocell, the macro BS is equipped with an MEC server, and MUs offload tasks to the MEC server through the small BSs. Fig.~\ref{Fig:Net_SingleServer} provides the pictorial illustration of these two network settings. The similarities of the aforementioned literature are in the assumption of the single MEC server and/or the fixed user association even in the case where an MU is under the coverage of multiple BSs. 

% width=0.36\linewidth
\begin{figure*}[!ht]
	\centering
	\subfloat[Single-cell and single-server MEC network. \label{Fig:HomNet_SingleServer}]{\includegraphics[width=0.38\linewidth]{./Images/HomNet_SingleServer.pdf}}\qquad 
	\subfloat[Multi-cell and single-server MEC network. \label{Fig:HetNet_SingleServer}]{\includegraphics[width=0.58\linewidth]{./Images/HetNet_SingleServer.pdf}}
	\caption{Two typical network settings of single-server MEC networks \cite{Pham2018MEC_HetNet}.}
	\label{Fig:Net_SingleServer}
\end{figure*}

\subsubsection{Single-server Het-MEC}
Merging MEC with the dense deployment of small-eNBs can provide many benefits; however, computation offloading and resource allocation schemes become very complicated due to the presence of inter-cell interference. There have been several papers working on interference management in dense Het-MEC systems \cite{Sardellitti2015Joint, AlShuwaili2017JointUplinkDownlink, Zhang2016EnergyEfficient, Zhang2018JointComputation, Zhao2018UplinkRA, Sun2017EMM}. In \cite{Sardellitti2015Joint}, the authors investigated a joint problem of radio and computational resources to minimize the total energy consumption of all mobile users under transmit power budget, latency, and maximum computing capability constraints. Because of the presence of inter-cell interference, the transmit covariance matrices of users are all coupled, thus resulting in a highly non-convex problem, even in the special case of a single user. With the aim of solving the original problem, two main approaches were considered \cite{Sardellitti2015Joint}. The first solution was to apply the idea of successive convex approximation (SCA), where the original problem was replaced by a sequence of strongly convex problems, while the other alternative was to decompose the original problem into subproblems that were solvable in parallel across the small-eNBs with limited signaling exchange between small-eNBs and the central cloud. Numerical simulation in \cite{Sardellitti2015Joint} showed that (1) the joint optimization was superior to disjoint schemes, where radio and computational resources were optimized separately and (2) computation tasks with high computational load and small number of bits were more beneficial from offloading and remote execution since the computing capability allocated to each offloading user is proportional to its computation task's workload. Similarly, Al-Shuwaili \textit{et al.} in \cite{AlShuwaili2017JointUplinkDownlink} considered several issues in single-server multi-cell Het-MEC systems: (1) the management of uplink and downlink interference, (2) the allocation of backhaul capacity for task offloading, and (3) the allocation of computing capabilities at the cloud for offloading users. In doing so, an optimization problem to optimize the uplink/downlink precoding, computation resource allocation, and uplink/downlink backhaul allocation was considered and then solved based on the SCA method. Simulation in \cite{AlShuwaili2017JointUplinkDownlink} showed the effectiveness of joint allocations of computing and backhaul resources and demonstrated the importance of backhaul capacity over the offloading energy consumption. 

In the presence of multiple users, the MEC server must be able to simultaneously execute multiple computation tasks and the scarce wireless bandwidth needs to be shared among multiple users. Compared to the resourceful cloud, the MEC server usually has finite resources and would not be able to meet all users’ computation requirements. As a consequence, the joint optimization of offloading decisions and resource allocation is an important research problem in MEC systems to improve the network performance \cite{Pham2018Mobile}. This joint optimization has been widely investigated in the literature \cite{Pham2018Mobile, Zhang2016EnergyEfficient, Zhang2018JointComputation}. Zhang \textit{et al.} proposed a three-step algorithm for solving the optimization problem of offloading decisions and radio resources in a HetNet with a macro-eNB, a small-eNB, and an MEC server. In the first step, users were divided into three groups, such as, ``offloading", ``local execution", and ``not specified". Next, based on the delay constraint, radio resources, and the offloading energy gain, different priorities were identified for users. Finally, the radio channels were allocated to mobile users based on their priorities. The algorithm proposed in \cite{Zhang2016EnergyEfficient} was an iterative scheme, where the second and third steps were iteratively updated until the convergence condition was satisfied. In \cite{Zhang2016EnergyEfficient}, there was a backhaul between the small-eNB and macro-eNB such that the computation offloading from users through the small-eNB incurs an extra delay due to the limited backhaul capacity. Different from \cite{Zhang2016EnergyEfficient}, Pham \textit{et al.} in \cite{Pham2018Mobile} optimized the offloading decisions, backhaul partitioning factor between wireless access and wireless backhaul transmissions, and computing resources at the MEC servers. Due to the problem NP-hardness, the authors proposed an iterative algorithm, where the offloading decisions were found based on the idea of matching theory and the resource allocation problem is convex and decomposable. The result conducted in \cite{Pham2018Mobile} indicated that the bandwidth partitioning was of critical importance to computation offloading in MEC with wireless backhaul. Another study devoting for the joint problem of computation offloading and resource allocation was considered in \cite{Zhang2018JointComputation}. In term of resource type, the authors considered the uplink subchannel, transmit power of mobile users, and computation resource at the MEC server. Unlike \cite{Pham2018Mobile, Zhang2016EnergyEfficient}, the offloading strategy in \cite{Zhang2018JointComputation} was formulated as a distributed potential game. Based on the offloading decisions, two solutions were proposed for subchannel allocation: uniform zero frequency reuse method where there was no interference among users and fractional frequency reuse based on Hungarian method and graph coloring method, where interference among users was taken into consideration. 

In order to realize the potential benefits of dense Het-MEC networks, a new technical challenge is mobility management. According to \cite{Wang2017LocalizedMobility, Semiari2018Caching}, there are several key issues for mobility management in Het-MEC systems. First, users may experience frequent handover when they move across different small-size and small-coverage smallcells/ MEC servers, thus increasing the overhead and interrupting the MEC services. In fact, handovers allow users to transfer their connections from the source to target MEC server while maintaining continuous computations and ensuring QoS. However, frequent handovers among small-cell MEC servers can increase handover failures and may be unnecessary for high-mobility users \cite{LopezPerez2012Mobility}. Second, continuously performing handover measurements and processing, which is needed to discover new target MEC servers in dense Het-MEC systems, is power- and radio resource-consuming, especially for battery-limited users. Third, in traditional dense HetNets, handover decision is mainly based on the quality of radio signals between users and potential eNBs. Actually, it is not suitable to use traditional handover decision criteria for mobility management in dense Het-MEC systems because (i) using MEC services requires both radio and computation resources; and (ii) scarce radio spectrum needs to be shared between normal and MEC servers; (iii) new challenges exists in MEC systems such as heterogeneous computing capabilities and various computation workloads. In addition, due to the lack of future information, e.g., channel conditions, available computing resources, task arrivals, the offloading and handover decisions should be known without prior information and be optimized in a long-term manner \cite{Sun2017EMM}. 

Due to its critical importance, an extensive body of work has appeared
in the literature to address the challenges of mobility management in conventional dense HetNets \cite{Wang2017LocalizedMobility, Semiari2018Caching, LopezPerez2012Mobility, Prasad2013EnergyEfficient, Xenakis2014Mobility, Giust2015Distributed, Zhang2017NetworkSlicing, Qiao2017JointDeployment}. For example, two localized mobility management schemes for dense HetNets were proposed in \cite{Wang2017LocalizedMobility}, a cache-enabled mobility management framework in mmWave-microwave HetNets was studied in \cite{Semiari2018Caching}, various energy-efficient cell discovery techniques were discussed in \cite{Prasad2013EnergyEfficient}, a comprehensive review of mobility management was provided in \cite{Xenakis2014Mobility}, and the adoption of distributed mobility management was presented in \cite{Giust2015Distributed}. Although interesting, the body of work in \cite{Wang2017LocalizedMobility, Semiari2018Caching, LopezPerez2012Mobility, Prasad2013EnergyEfficient, Xenakis2014Mobility, Giust2015Distributed, Zhang2017NetworkSlicing, Qiao2017JointDeployment} solely focused on mobility management in HetNets. Taking challenges of mobility management in dense Het-MEC systems into consideration, the study in \cite{Sun2017EMM} optimized the association (which MEC server is selected for remote execution) and handover (i.e., when task migration is needed) decisions to minimize the average delay with the long-term energy budget constraint. Simulation in \cite{Sun2017EMM} indicated that without complete future information, the proposed algorithm for energy-efficient mobility management can still achieve close-to-optimal performance while guaranteeing the long-term energy budget constraint. 

\subsubsection{Multi-server Het-MEC}
The sever diversity in multi-server Het-MEC systems opens great opportunities for users to receive better MEC services but at the same time introduces new technical issues including server selection, server collaboration, and service migration \cite{Mao2017_aSurveyMEC}. 

\noindent \textit{a) Server selection:} When multiple MEC servers are available for remote computation, a key issue is the selection of the target server, which is similar to the concept of user association (UA) in dense HetNets. Presently, there exist two main directions for server selection: (i) \textit{user association} when a mobile user is under the coverage range of multiple MEC servers and (ii) \textit{server selection} when the cooperation of MEC and cloud servers is needed to process heterogeneous computations. In \cite{Dinh2017Offloading}, the joint problem of local CPU frequency and computation offloading was studied for MEC systems with a single user and multiple MEC servers. The objective was to minimize the computation overhead, which was defined as the weighted sum of total energy consumption and execution latency, and the constraints ensure that each computation task can be handled by only one MEC server. Due to the problem NP-hardness, the exhaustive search method was used to find the optimal solution while a semidefinite relaxation-based approach was proposed to find the near optimal solution in polynomial time and with low complexity. Tran \textit{et al.} in \cite{Tran2018JointTaskOffloading} explored the problem of server selection and resource allocation, where resources were subchannel used to offload computations to the target server, transmit power of mobile users, and computing resources at the MEC servers. The main challenges arised from binary computation offloading and subchannel assignment, which made the optimization problem NP-hard. To cope with these issues, the authors decomposed the underlying problem into two smaller problems of computation offloading and resource allocation and proposed solving these two subproblems by a new heuristic method and the convex optimization technique, respectively. The simulation results reported that the consideration of multiple MEC servers, even in the presence of inter-cell interference, can improve the performance compared to the scheme, where the computation offloading and resource allocation were optimized independently at each MEC server. This work was further improved in \cite{Pham2018Decentralized}, where the offloading decisions and subchannel assignment were achieved by using the matching theory. It was shown that the proposed algorithm can find the offloading decisions in a distributed manner while still guaranteeing the solution convergence and performance gap. More recently, other relevant studies have been conducted in small-cell networks with MEC, for example, the combination of genetic algorithm and particle swarm optimization was utilized to solve the joint problem of offloading decision and resource allocation in \cite{Guo2017EnergyEfficient, Guo2018AnEfficient} and a distributed offloading scheme was investigated in \cite{Yang2018ADistributed}. 

Inspired by the fact that MEC and MCC are two complementary technologies, several recent works were proposed to tackle the shortcomings of each computing paradigm and further enhance the user performance from the perspective of computation offloading \cite{Guo2018Collaborative, Guo2018CollaborativeMECO}. In \cite{Guo2017Collaborative, Guo2018Collaborative, Guo2018CollaborativeMECO}, a general architecture of hybrid fiber-wireless (FiWi) networks for the coexistence of centralized cloud and distributed MEC servers was proposed. Specifically, a FiWi network comprises two parts, including (1) the optical backhaul connecting between users and the central cloud and (2) the front end segment providing wireless accesses for users. Moreover, adopting the proposed network architecture, the authors investigated a collaborative computation offloading scheme, where computations can be offloaded to either the distributed MEC server or the centralized cloud server. The design of FiWi networks with MEC capabilities was generalized in \cite{Rimal2017MEC}. For the illustration of MEC over FiWi networks, discussions with three typical RAN technologies in the wireless front (wireless local area network, 4G LTE, LTE-A HetNets) end were provided. In addition, a two-layer time-division multiplexing based resource allocation scheme for the coexistence of H2H and MEC traffic was proposed, where the first layer was designed for the optical backhaul segment and the second layer schedules transmissions of mobile users. Some recent works extended the study in \cite{Rimal2017MEC} for resource management \cite{Rimal2017Cloudlet, Rimal2017MECversusCentralizedCC}, a virtualized FiWi network with MEC \cite{Liu2018PerformanceEvaluation}, the proof-of-concept demonstration \cite{Rimal2018ExperimentalTestbed}, and a novel MEC architecture for IoT \cite{Ansari_IEICE18}. Other recent studies in \cite{Chen2016JointOffloading, Chen2018Resource, Chen2018MultiUser} derived the offloading decision and resource allocation in a three-tier MEC setting with an MEC server and a remote cloud. Specifically, in \cite{Chen2016JointOffloading} an optimization problem was formulated to minimize the total system cost that was defined as the weighted sum of the total energy consumption, the offloading and processing costs, and the transmission and processing delays. This problem was extended in \cite{Chen2018Resource} for multi-user MEC settings and in \cite{Chen2018MultiUser} for multi-user multi-task scenarios. Since the considered problems were all non-convex, thus generally NP-hard, the offloading decision was solved by heuristic algorithms, which were designed based on semidefinite relaxation and a randomization mapping method 

\noindent \textit{b) Server collaboration:} Conventionally, the MEC concept does not describe the collaboration and synergy among different MEC servers. Due to the limited resource of each MEC server, it is hard to handle all of the compute-intensive tasks from a large number of mobile users by only one single server \cite{Ndikumana2019JointCommunication}. Computations that exceed the MEC server's maximum computing capability have to be offloaded to the centralized cloud, thus incurring extra latency and computation overhead. Therefore, relying on individual MEC for computation can limit the performance of MEC systems. Recently, several research works focusing on collaborative MEC have been proposed in the literature \cite{Tran2017Collaborative, Tran2017CollaborativeMultiBitrate, Wang2018EnablingMEC}. In \cite{Tran2017Collaborative, Tran2017CollaborativeMultiBitrate}, three case studies of MEC were presented to demonstrate the benefits of collaboration among MEC servers, including mobile edge orchestration, collaborative video caching and processing, and two-layer interference cancellation. The authors also provided some challenges and open research issues in collaborative MEC such as resource management, interoperability among different MEC infrastructure providers, and service discovery and synchronization. Wang \textit{et al.} in \cite{Wang2018EnablingMEC} proposed a novel edge computing framework for vehicular networks. Since SDN offers many advantages, e.g., the low cost for deployment and development of new services, the global knowledge of the network state, and the ability to control in a vendor-independent manner, the authors proposed using SDN to control the operations of collaborative MEC. To make the concept of MEC collaboration a reality, NFV, SDN, smart collaborative networking, and blockchain were identified as three enabling technologies of the collaborative vehicular edge computing framework. 

More recently, Ndikumana \textit{et al.} in \cite{Ndikumana2019JointCommunication} indicated that a variety of issues and challenges emerge in MEC systems when dealing with big data and edge analytics: (i) users offload their computation tasks and corresponding to the MEC server with either finite or infinite flow, (ii) collaboration among nearby MEC servers is needed to reduce the data exchange between users and the remote cloud and handle big data, and (iii) a new model that integrates communication, computation, caching, and control is required for big data MEC. To address these challenges, the authors first proposed a new algorithm for grouping MEC servers into different collaboration spaces, that was based on the overlapping k-mean method \cite{Cleuziou2008AnExtended}. Within each cluster, an optimization problem was formulated to maximize the bandwidth saving and minimize the total delay, which was difficult to solve because of its non-convexity. Instead of solving the problem optimally, a block successive upper bound minimization (BSUM) was applied to achieve a sub-optimal solution that was able to converge with sub-linear convergence speed. This work was extended in \cite{Ndikumana2018DeepLearning} for self-driving car, where MEC servers are deployed at roadside units (RSUs). It was shown that the proposed algorithms in \cite{Ndikumana2019JointCommunication, Ndikumana2018DeepLearning} can reduce the total delay compared with the existing schemes. Based on the concept of collaborative MEC, several studies have been proposed recently, for example, a collaborative cache allocation and computation offloading, where MEC servers collaborate with nearby neighbors for executing computations and caching \cite{Ndikumana2017CollaborativeCache}, an adaptive bitrate video (ABR) caching and processing scheme, where an MEC server collaborates with others for both caching and transcoding ABR videos \cite{Tran2018AdaptiveBitrate}, a novel survivable virtual network embedding framework for collaborative edge computing in smart cities \cite{Hou2018GreenSurvivable, Gong2017VirtualNetwork}, and a socially-trusted platform for ultra-dense edge computing networks, where users are allowed to select the target small-eNB and the security-aware incentive collaboration among MEC servers was designed based on the coalitional game theoretic framework \cite{Chen2017SociallyTrusted}. 

\noindent \textit{c) Service migration:} A critical problem in MEC systems is dynamics at the network edge, which are mainly caused by the user mobility and limited coverage of small-scale MEC servers. When a mobile user moves from the service coverage of the source MEC server to others, there are two options to ensure the service continuity \cite{Wang2014Mobility}: (1) migrate computations from the source MEC server to the target server that is near the current user location and (2) continue executing the computations on the source MEC server and then forward the result to users via the target MEC server. One the one hand, computation migration has the advantages of guaranteeing the MEC service continuity and improving the user QoS (e.g., lower latency). On the other hand, one has to pay some extra cost for computation migration, e.g., migration execution cost, incentive payment to the target MEC server, and transmission cost due to radio resource usage. Several challenges arise in computation migration due to the following reasons \cite{Wang2018aSurvey}. First, when should the computation task be migrated from the source server? Next, which is the target server to execute the task when a computation is needed? This problem becomes very challenging since the ultra-dense deployment of small-scale MEC servers is expected in 5G networks and beyond. Last, how to process computation migration? This is critical when various QoS requirements are taken into consideration and the tradeoff between QoS improvement and migration cost is considered. The principle of computation migration is illustrated in Fig.~\ref{Fig:ComputationMigration}, where the mobile user is initially offloaded to the source MEC server. When the user moves to a new location that is close to the new server, the computation migration from the source to target MEC server is to ensure the MEC service continuity. 

\begin{figure} [ht]
	\centering
	\includegraphics[scale=0.65]{./Images/ComputationMigration.pdf}
	\caption{Illustration of computation migration.}
	\label{Fig:ComputationMigration}
\end{figure}


Motivated by potential benefits, several studies have been carried out for computation migration in Het-MEC systems over the last few years. The problem of computation migration for an MEC system with a single user and multiple MEC servers was formulated as a Markov decision process (MDP) \cite{Ksentini2014aMDP}, where the mobile user followed a 1-D asymmetric random walk mobility model. While the optimal policy of the proposed problem was solved by standard algorithms for MDP in \cite{Ksentini2014aMDP}, which was later extended in \cite{Wang2014Mobility} to derive a threshold policy-based mechanism, in \cite{Wang2015DynamicService} to consider general cost models, 2-D mobility model, and application to real-world traces, and in \cite{Wang2017DynamicService} to remove the Markovian assumption and deal with dynamic service arrivals and departures. In \cite{Machen2018LiveServiceMigration}, a three-layer framework was proposed for computation migration in MEC. The traditional framework includes two layers that are the base layer and the instance layer while an additional application layer, which has an idle version of the application and any application-specific data, was introduced in order to reduce the migration downtime. The main advantage of the proposed three-layer was that it was designed based on existing technologies (e.g., virtual machines and containers) so that new computation migration can be fastly deployed without any internal modification. For more details of service migration in edge computing, interested readers may refer to the recent survey paper \cite{Wang2018aSurvey}. 


\subsection{Learned Lessons and Potential Works}
\label{SubSec:Lesson_and_Potential_Works_HetNet}
Due to the great benefits offered by MEC and HetNet as well as their complementary properties, it is convinced that the combination of MEC and dense HetNet is unavoidable in the future. Although various problems and issues in dense Het-MEC systems have been intensively studied, there are still several challenges. In the following, we discuss some challenges in dense Het-MEC systems and outline the open research directions. 
\begin{itemize}
	\item \textit{Computational complexity and signaling overhead}: Obviously, centralized optimization is usually easy to implement compared to distributed approaches and can provide the optimal/near-optimal solution with the desired performance guarantee. However, such centralized approaches are not scalable due to the explosive increase in the number of mobile users, eNBs, and MEC servers. As a result, there is a need for lightweight and effective algorithms. In these schemes, distributed approaches can offer many benefits as it does not need any central entity and the algorithms are based on only local information or small amounts of signaling overhead. However, it is hard to guarantee the solution optimality with distributed approaches due to the lack of complete information. Therefore, one needs to tradeoff between the computational complexity and solution optimality. An effective way is to decompose the entire network into several regions and assign the responsibility for executing the algorithm to distributed MEC servers, that is the underlying problem is decomposed into subproblems, which are executed distributively at different MEC servers. This would significantly reduce the amount of information which need to be exchanged between the central entity and all users; hence, the network overhead can be also degraded. 
	\item \textit{Mobility management}: Ensuring the benefits of mobile users through computation offloading while taking into account user mobility is a challenging issue. Most existing studies in (dense Het-) MEC systems ignore the effect of user mobility due to its difficulty and intractability. Because of mobility, users may change their positions while using MEC services, e.g., they can move out of the coverage area of their source MEC servers and are in the serving coverage of other ones. In this case, MEC needs to be aware of user mobility in order to maintain service continuity. This is important since there are various types of users with different mobility levels including static users (e.g., environmental sensors), low-mobility users (e.g., pedestrian users), and high-mobility users (e.g., express trains). One potential solution to deal with user mobility is enabling MEC servers to continuously update the user context and then designing context-aware algorithms. Instead of using one-shot optimization, long-term optimization can be used to tackle the challenges of user mobility. To illustrate this point, we consider the following example with a mobile user, which is located far from the MEC server. The short-term optimization for computation offloading decision is not offloading, that is local execution. However, fixing this short-term decision is not always optimal since the user can move to a new position with better channel quality. Moreover, the short-term offloading decision affects not only the instant performance but also the long-term energy budget. In summary, there is a big room for researches into mobility management in dense Het-MEC systems. 
	\item \textit{Interference management}: Inherited from dense HetNets, the challenges for interference management in dense Het-MEC systems remain to be solved for many reasons. First, the ultra-dense deployment of users, eNBs, and MEC severs make the distance between any two points shorter; therefore, interference becomes more severe, thus lowering the overall performance. Second, heterogeneity of mobile users and MEC servers makes the interference problem more challenging due to various transmit power budget of users in the uplink and of MEC servers in the downlink. Next, the various computation task characteristics require different priorities for users in accessing radio and MEC resources. Finally, interference management is highly coupled with other domains, such as resource allocation and network planning. Hence, more sophisticated interference management schemes incorporating features of dense HetNets and MEC systems would be highly required for improving the users QoS with MEC services. \\
	\item \textit{Wireless Backhaul}: Most of the research works on Het-MEC share the assumption of wired backhaul links between any two small-eNB and macro-eNB, thus ignoring the backhaul transmission latency. At the time of paper writing, there is only one study focusing on MEC with wireless backhaul \cite{Pham2018Mobile}; however, the network setting in this literature is simple, comprising a small-eNB and an MEC server collocated at the macro-eNB. This work is served as a fundamental study for more complex frameworks, e.g., the extension to dense Het-MEC systems and the consideration of mixed wireless and wired backhaul links.
\end{itemize}
